Modeling Collaboration in Academia: A Game Theoretic Approach

In this work, we aim to understand the mechanisms driving academic collaboration. We begin by building a model for how researchers split their effort between multiple papers, and how collaboration affects the number of citations a paper receives, supported by observations from a large real-world publication and citation dataset, which we call the h-Reinvestment model. Using tools from the field of Game Theory, we study researchers' collaborative behavior over time under this model, with the premise that each researcher wants to maximize his or her academic success. We find analytically that there is a strong incentive to collaborate rather than work in isolation, and that studying collaborative behavior through a game-theoretic lens is a promising approach to help us better understand the nature and dynamics of academic collaboration.

==> 05-conclusions.tex <==

\section{Conclusions and Future Work}
\label{sec:conclusions}

In this work, we have presented a game-theoretic approach to studying collaborative behavior in academia by modeling research\-ers as rational agents trying to maximize their academic success. Several publication models have been proposed in the literature, but to our knowledge, ours is the first with the flexibility to model collaborative behaviors that may change over time in response to actions of and interactions with others.

Many modifications and extensions to our model are possible. For example, instead of all decisions being deterministic, one could allow
mixed strategies, where a player's action in a year is selected from a distribution over possible strategies. Also, our analysis was performed under the premise that researchers want to maximize their h-index. In previous work we introduced the Social h-index, which aims to capture not only the direct impact of a researcher on the research corpus, but also on his or her fellow researchers~\cite{CMMT@JOI13}. It is natural to study the game where the object is to maximize such variant measures.

The policies of our academic institutions, as well as the unspoken rules and expectations of academia, inevitably shape the mentalities and goals of individual researchers, encouraging certain behaviors and discouraging others. An increased ability to understand the effects of these motivating forces will help policy-makers and academic leaders to make informed decisions that will stimulate the growth and progress of the academic community.


%%%%%%%%%%

%Here we consider two variants, the Instantaneous Social h-index and the Progressive Social h-index.

%Taking the h-index as a suitable metric for the impact of a person's individual research contributions, we define the {\em Social h-index} of author $a$ to be
%$$\sum_{p \in P(a)} \frac{1}{|A(p)|} \sum_{a' \in A(p)} \cont(p,a'),$$
%where $\cont(p,a')$ measures how much paper $p$ has contributed to the h-index of $a'$. That is, for each paper $a$ has coauthored, he gets partial credit for the contribution of that paper to each coauthors' h-index, including himself. We suggest two instantiations of the $\cont$ function, one based on whether the paper currently contributes to a designated author's h-index, and the other which considers its cumulative contribution over time.

%For the {\em Instantaneous Social h-index} of author $a$, denoted $\inst(a)$, we define
%\begin{equation*}
%	\cont(p,a) =
%	\begin{dcases*}
%		\frac{h(a)}{\abs{H(a)}} & if $p \in H(a)$ \\
%		0 & otherwise
%	\end{dcases*}
%\end{equation*}
%A natural first thought would have been to set $\cont(p,a) = 1$ if $p \in H(a)$ and $0$ otherwise. However, due to ties, we may have $\abs{H(a)} > h(a)$. The above definition maintains the property that $\sum_{p \in P(a)} \cont(p,a) = h(a)$, even in the case of ties. Note that it is possible for $\cont(p,a)$ as defined above to decrease over time, e.g. if $a$ publishes additional papers which bring $h(a) > cit(p)$. Next, we suggest a version of the Social h-index which is non-decreasing.

%For each $i \leq h(a)$, consider the time at which $a$ first achieved an h-index of $i$, and let $H^{(i)}(a) \subseteq P(a)$ be the set of papers with at least $i$ citations at that time. For the {\em Progressive Social h-index} of author $a$, denoted $\prog(a)$, we define
%\begin{equation*}
%	\cont(p,a) = \sum_{\substack{i \leq h(a) \colon \\ p \in H^{(i)}(a)}} \frac{i}{|H^{(i)}(a)|}.
%\end{equation*}
%Intuitively, the Progressive Social h-index assigns partial credit to a researcher's coauthors every time her h-index increases. We note that $\prog(a)$ is non-decreasing over time. That is, once $a$ gets credit for contributing to another's success, that credit can not be overshadowed by future work. However, an exceptionally good paper could continue reaping rewards as a coauthor's h-index grows, if it remains one of the contributing papers.

%Future work could analyze the AC game using the Instantaneous or the Progressive Social h-index as the players' utility functions, and compare the resulting behavior with that in the current work. Furthermore, while we focused on the context of academia, our approach can be applied to study collaborative behavior in other contexts such as business teams and collaborative design.

%Practicality: Compare the complexity (in terms of time, space, and ease of acquiring data) of computing h, soc-h, and prog-soc-h. We show that the Progressive Social h-index can be updated dynamically. Suppose we have calculated...
%analyze the impact this behavior has on the research community as a whole
%social g, etc.

